Nominal Unification Revisited

Nominal unification calculates substitutions that make terms involving binders equal modulo alpha-equivalence. Although nominal unification can be seen as equivalent to Miller's higher-order pattern unification, it has properties, such as the use of first-order terms with names (as opposed to alpha-equivalence classes) and that no new names need to be generated during unification, which set it clearly apart from higher-order pattern unification. The purpose of this paper is to simplify a clunky proof from the original paper on nominal unification and to give an overview over some results about nominal unification.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Maribel Fernandez (Ed.): 24th International Workshop on \\ Unification (UNIF2010).\\
EPTCS 42, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.42.1}{10.4204/EPTCS.42.1}}
\pdfoutput=1

